Graph-based 3D Collision-distance Estimation Network with Probabilistic Graph Rewiring

We aim to solve the problem of data-driven collision-distance estimation given 3-dimensional (3D) geometries. Conventional algorithms suffer from low accuracy due to their reliance on limited representations, such as point clouds. In contrast, our previous graph-based model, GraphDistNet, achieves high accuracy using edge information but incurs higher message-passing costs with growing graph size, limiting its applicability to 3D geometries. To overcome these challenges, we propose GDN-R, a novel 3D graph-based estimation network.GDN-R employs a layer-wise probabilistic graph-rewiring algorithm leveraging the differentiable Gumbel-top-K relaxation. Our method accurately infers minimum distances through iterative graph rewiring and updating relevant embeddings. The probabilistic rewiring enables fast and robust embedding with respect to unforeseen categories of geometries. Through 41,412 random benchmark tasks with 150 pairs of 3D objects, we show GDN-R outperforms state-of-the-art baseline methods in terms of accuracy and generalizability. We also show that the proposed rewiring improves the update performance reducing the size of the estimation model. We finally show its batch prediction and auto-differentiation capabilities for trajectory optimization in both simulated and real-world scenarios.

==> 4_2_Method.tex <==
\section{Methodology Enhancement}\label{sec_method_enhancement}
\subsection{Prior score module}
Though we benefit from a rewiring strategy, it cannot guarantee to sample $i^*$ since regardless of the convergence, we have a limited number of layers.
To compensate for this limitation, we exploit the prior score module for better initial node selection.
Goal position given from \cite{you2021omnihang} benchmark dataset, we generate path set $T_{o_1, o_2} = \{ \tau_1, \tau_2, ..., \tau_{K} \}$ with length K.
We randomly selected the start position and $\tau$ represents a 7-dimensional relative transformation vector.
 We use rapidly exploring random tree (RRT) for path generation.
For each category of objects (cap, mug, hook, etc), we have variations in a particular category.
For simplicity, let's say in the case of cap, we have an object set of $\{ cap_1, cap_2, cap_3, ...\}$ for the cap category \ref{fig:collection}.
We collect hanging paths for each object variant.
For cap1, $RRT_{cap_1}$ is composed with $RRT_{cap_1, hook_1}$, $RRT_{cap_1, hook_2}$, and $RRT_{cap_1, hook_H}$ where H refers to the variation number of hook.
For each $RRT_{cap_1, hook_h}$, there exists number L=10 number of RRT paths $RRT_{cap_1, hook_h} = \{ T^1_{cap_1, hook_h}, T^2_{cap_1, hook_h}, ...T^L_{cap_1, hook_h}\}$.
Utilizing this RRT path for a particular object as prior knowledge for collision, we create an object-specific score per each object $S_{cap1}$ as follows
\begin{align}
    S_{obj} = \rho\left(
    \sum_{\substack{l=1...L \\\ h=1...H}}
    \triangle\left( g \left( \mathcal{V}_{obj}, T^l_{obj, h} \right), \mathcal{V}_{h} \right)
    \right),
\end{align}

% $ S_{o} = normalize\left( \triangle\left( g \left( P_{obj}, \tau_{k} \right), P_{hook} \right) \right)$. 
where $\triangle\left(\cdot,\cdot\right)$ represents vertex-wise Euclidean distance and $g$ is a function that calculates transformation with a given 7-dof transformation vector.
$\rho$ is a normalization function that maps values to [0, 1].
In this work, we utilize the softmax function.
We use these score values as labels for score module training.
Exploiting Pointnet \cite{qi2017pointnet++} structure as an embedding module, we optimize the score-predicting module with given vertices set $\mathcal{V}_{obj}$.
We regard each vertex from the graph structure as a point cloud.
% To preserve the initial position, we set the query radius to 0.0. 
% For multiple sampled pose, we stack scores $S_{collision}^{1,..,K} \in \mathbb{R}^{K}$ 

For feature encoding, we use Pointnet \cite{qi2017pointnet}.
During training, we use binary classification with logits error as a loss so that the model is optimized with respect to the node-wise probability.
After training, the model returns each node's probability about the collision awareness.
From this probability distribution, we sample key points with a fixed number of 8.
To prevent dense or sparse keypoint selection, we apply relaxed softmax before the sampling procedure with a temperature value of $0.5$.
We use the alias method multinomial sampling that is implemented in the Pytorch library.

\subsection{Gradient estimation for trajectory optimization}
Unlike collision estimators \cite{son2023local}, \cite{murali2022cabinet} that return boolean results of whether there is a collision or not, our model returns continuous distance value of collision distance $\Tilde{d}$.
Using automatic differentiation tools in deep learning such as Pytorch, we can compute the gradient of distance with respect to an object's joint configuration.
% We assume grasped object by a robot gripper attached to the manipulator. 
From this, we can estimate the gradient of the manipulator's joint configuration.
This setting is similar to that of \cite{kim2022graphdistnet}, \cite{zhi2022diffco}.


\begin{figure}
 \center
  \includegraphics[width=\linewidth]{images/prior2.pdf}
  \caption{
    Results of the prior model with diverse categories of objects. Our prior model gets the object's mesh vertices as input and returns the probability of the collision-aware key point while hanging the object.
  }
  \label{fig:prior}
    \vspace{-0.5em}
\end{figure}

==> 8_Future_Work.tex <==
\section{Future Works}
\mj{There exists several avenues of improvement in our method. First, during the trajectory optimization step, we did not perform batch computation. We hope to show the superior performance of our methods quantitatively in the next project. Second, dynamic collision distance estimation in the 4D temporal domain is another challenging point. We hope our method can be applied to the continuous collision distance estimation problem.}
